When and Why Adversarial Training Improves PINNs: A Neural Tangent Kernel Perspective

Physics-informed neural networks (PINNs) are powerful surrogates for differential equations but are notoriously difficult to train due to spectral bias, stiffness, and poor accuracy on high-frequency or multiscale solutions. Adversarial training based on generative adversarial networks (GANs) has recently gained surprisingly strong empirical results in improving training, but the underlying mechanisms remain elusive. To this end, we propose a new analysis framework for adversarially trained PINNs, based on the key observation of how the discriminator in GANs can influence the training dynamics of PINNs. The framework first provides a much needed theoretical grounding to why and when adversarial training is effective in PINNs, then presents a unified analysis of GANs variants in such training, and finally leads to a new, practical, efficient training algorithm for PINNs. Empirical results demonstrate that our method can significantly reduce the pathology of PINNs training, thereby providing better models with superior performances, often several magnitudes more accurate than alternative methods.

==> preambles.tex <==
%% This file contains a number of tweaks that are typically applied to the main document.
%% They are not enabled by default, but can be enabled by uncommenting the relevant lines.

%%
%% Inline annotations; for predefined colors, refer to "dvipsnames" in the xcolor package:
%% https://tinyurl.com/overleaf-colors
%%

\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{blue}[TODO: #1]}}
\newcommand{\HW}[1]{\textbf{\color{red}[HW: #1]}}
\newcommand{\added}[1]{\textcolor{green!60!black}{#1}}
\newcommand{\removed}[1]{\textcolor{red!70!black}{\sout{#1}}}

\RequirePackage{times}    % Integrate Times for here
\RequirePackage{xspace}
\RequirePackage[dvipsnames]{xcolor}
\RequirePackage{graphicx}
\RequirePackage{amsmath}
\RequirePackage{booktabs}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} \def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\iid{i.i.d\onedot} \def\wolog{w.l.o.g\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother


\newcommand{\mat}[1]{\mathbf{#1}}


\AtEndPreamble{
    \usepackage[capitalize]{cleveref}
    \crefname{section}{Sec.}{Secs.}
    \Crefname{section}{Section}{Sections}
    \Crefname{table}{Table}{Tables}
    \crefname{table}{Tab.}{Tabs.}
}

%%
%% disable for camera ready / submission by uncommenting these lines  
%%
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

%%
%% work harder in optimizing text layout. Typically shrinks text by 1/6 of page, enable
%% it at the very end of the writing process, when you are just above the page limit
%%
% \usepackage{microtype}

%%
%% fine-tune paragraph spacing
%%
% \renewcommand{\paragraph}[1]{\vspace{.5em}\noindent\textbf{#1.}}

%%
%% globally adjusts space between figure and caption
%%
% \setlength{\abovecaptionskip}{.5em}


%%
%% Allows "the use of \paper to refer to the project name"
%% with automatic management of space at the end of the word
%%
% \usepackage{xspace}
% \newcommand{\paper}{ProjectName\xspace}

%%
%% Commonly used math definitions
%%
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}

%%
%% Tigthen underline
%%
% \usepackage{soul}
% \setuldepth{foobar}

\usepackage{booktabs}
\usepackage{colortbl}
\usepackage{tabularx}
\usepackage{multirow}

\usepackage{enumitem}
\setlist[itemize]{noitemsep, topsep=2pt, parsep=0pt, partopsep=0pt}
\setlist[enumerate]{noitemsep, topsep=2pt, parsep=0pt, partopsep=0pt}

\setlength{\textfloatsep}{12pt}
\setlength{\floatsep}{12pt}
\setlength{\intextsep}{12pt}
\setlength{\tabcolsep}{3pt}

\setlength{\abovecaptionskip}{4pt}
\setlength{\belowcaptionskip}{0pt}

% Define colors
\definecolor{best}{HTML}{D5E8D4} %Light Green 
\definecolor{second}{HTML}{FFF2CC} % Light Yellow 

\newcommand{\colw}{0.135\textwidth}
%\newcommand{\figrow}[2]{%
%    \textbf{#1}\par\vspace{2pt}
%    \includegraphics[width=\colw]{#2/1.png}
%    \includegraphics[width=\colw]{#2/2.png}
%    \includegraphics[width=\colw]{#2/3.png}
%    \includegraphics[width=\colw]{#2/4.png}
%    \includegraphics[width=\colw]{#2/5.png}
%    \includegraphics[width=\colw]{#2/6.png}
%    \includegraphics[width=\colw]{#2/gt.png}
%    \par\vspace{6pt}
%}

\newcommand{\figrow}[2]{%
    \textbf{#1}\par\vspace{1pt}

    \begin{minipage}{\colw}\centering
        \includegraphics[width=\linewidth]{#2/4dgs_iclr.png}\\[0.01\linewidth]
        \includegraphics[width=0.49\linewidth]{#2/4dgs_iclr_a.png}\hfill
        \includegraphics[width=0.49\linewidth]{#2/4dgs_iclr_b.png}
    \end{minipage}
    \begin{minipage}{\colw}\centering
        \includegraphics[width=\linewidth]{#2/4dgs_cvpr.png}\\[0.01\linewidth]
        \includegraphics[width=0.49\linewidth]{#2/4dgs_cvpr_a.png}\hfill
        \includegraphics[width=0.49\linewidth]{#2/4dgs_cvpr_b.png}
    \end{minipage}
    \begin{minipage}{\colw}\centering
        \includegraphics[width=\linewidth]{#2/ex4dgs.png}\\[0.01\linewidth]
        \includegraphics[width=0.49\linewidth]{#2/ex4dgs_a.png}\hfill
        \includegraphics[width=0.49\linewidth]{#2/ex4dgs_b.png}
    \end{minipage}
    \begin{minipage}{\colw}\centering
        \includegraphics[width=\linewidth]{#2/ftgs.png}\\[0.01\linewidth]
        \includegraphics[width=0.49\linewidth]{#2/ftgs_a.png}\hfill
        \includegraphics[width=0.49\linewidth]{#2/ftgs_b.png}
    \end{minipage}
    \begin{minipage}{\colw}\centering
        \includegraphics[width=\linewidth]{#2/graphigs.png}\\[0.01\linewidth]
        \includegraphics[width=0.49\linewidth]{#2/graphigs_a.png}\hfill
        \includegraphics[width=0.49\linewidth]{#2/graphigs_b.png}
    \end{minipage}
    \begin{minipage}{\colw}\centering
        \includegraphics[width=\linewidth]{#2/graphits.png}\\[0.01\linewidth]
        \includegraphics[width=0.49\linewidth]{#2/graphits_a.png}\hfill
        \includegraphics[width=0.49\linewidth]{#2/graphits_b.png}
    \end{minipage}
    \begin{minipage}{\colw}\centering
        \includegraphics[width=\linewidth]{#2/gt.png}\\[0.01\linewidth]
        \includegraphics[width=0.49\linewidth]{#2/gt_a.png}\hfill
        \includegraphics[width=0.49\linewidth]{#2/gt_b.png}
    \end{minipage}

    \par\vspace{1pt}
}

% ===== SPLIT LAYOUT (4 items top, 3 items bottom) =====
\newcommand{\figrowSplit}[1]{%

  \def\sw{0.24\linewidth}%
  
  % --- ROW 1: Competitors (4 items) ---
  \begin{minipage}[t]{\sw}\centering\scriptsize 4DGS-1 \cite{yang2023gs4d}\par\vspace{1pt}
    \includegraphics[width=\linewidth]{#1/4dgs_iclr.png}\\[0.01\linewidth]
    \includegraphics[width=0.49\linewidth]{#1/4dgs_iclr_a.png}\hfill
    \includegraphics[width=0.49\linewidth]{#1/4dgs_iclr_b.png}
  \end{minipage}\hfill
  \begin{minipage}[t]{\sw}\centering\scriptsize 4DGS-2 \cite{wu20244d}\par\vspace{1pt}
    \includegraphics[width=\linewidth]{#1/4dgs_cvpr.png}\\[0.01\linewidth]
    \includegraphics[width=0.49\linewidth]{#1/4dgs_cvpr_a.png}\hfill
    \includegraphics[width=0.49\linewidth]{#1/4dgs_cvpr_b.png}
  \end{minipage}\hfill
  \begin{minipage}[t]{\sw}\centering\scriptsize Ex4DGS \cite{lee2024fully}\par\vspace{1pt}
    \includegraphics[width=\linewidth]{#1/ex4dgs.png}\\[0.01\linewidth]
    \includegraphics[width=0.49\linewidth]{#1/ex4dgs_a.png}\hfill
    \includegraphics[width=0.49\linewidth]{#1/ex4dgs_b.png}
  \end{minipage}\hfill
  \begin{minipage}[t]{\sw}\centering\scriptsize FTGS \cite{wang2025freetimegs}\par\vspace{1pt}
    \includegraphics[width=\linewidth]{#1/ftgs.png}\\[0.01\linewidth]
    \includegraphics[width=0.49\linewidth]{#1/ftgs_a.png}\hfill
    \includegraphics[width=0.49\linewidth]{#1/ftgs_b.png}
  \end{minipage}
  
  \par\vspace{6pt} % Gap between top and bottom rows
  
  % --- ROW 2: Ours + GT (3 items, Centered) ---
  {\centering
  \begin{minipage}[t]{\sw}\centering\scriptsize \textbf{Ours (GraphiGS)}\par\vspace{1pt}
    \includegraphics[width=\linewidth]{#1/graphigs.png}\\[0.01\linewidth]
    \includegraphics[width=0.49\linewidth]{#1/graphigs_a.png}\hfill
    \includegraphics[width=0.49\linewidth]{#1/graphigs_b.png}
  \end{minipage}\hspace{2mm} % Slight gap
  \begin{minipage}[t]{\sw}\centering\scriptsize \textbf{Ours (GraphiTS)}\par\vspace{1pt}
    \includegraphics[width=\linewidth]{#1/graphits.png}\\[0.01\linewidth]
    \includegraphics[width=0.49\linewidth]{#1/graphits_a.png}\hfill
    \includegraphics[width=0.49\linewidth]{#1/graphits_b.png}
  \end{minipage}\hspace{2mm} % Slight gap
  \begin{minipage}[t]{\sw}\centering\scriptsize GT\par\vspace{1pt}
    \includegraphics[width=\linewidth]{#1/gt.png}\\[0.01\linewidth]
    \includegraphics[width=0.49\linewidth]{#1/gt_a.png}\hfill
    \includegraphics[width=0.49\linewidth]{#1/gt_b.png}
  \end{minipage}
  \par}
}

\newcommand{\figrowCrops}[1]{%
  % Configuration
  \setlength{\tabcolsep}{1pt} % Minimal horizontal gap
  \renewcommand{\arraystretch}{0.5} % Minimal vertical gap
  
  % --- Left Block: Full Ground Truth ---
  \begin{minipage}[c]{0.28\linewidth} 
    \centering
    % Label in 2 lines to match the height of headers on the right
    \parbox{2.5cm}{\centering \scriptsize \textbf{Ground}\\\textbf{Truth}} \par\vspace{3pt}
    \includegraphics[width=\linewidth]{#1/gt.png}
  \end{minipage}%
  \hfill % Push grid to right
  % --- Right Block: 6 Columns of Methods ---
  \begin{minipage}[c]{0.71\linewidth}
    \centering
    \tiny % Use tiny text to fit method names
    \begin{tabular}{@{}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{}}
      % --- Header Row: Method Names ---
      % Note: I used \parbox on the left label, so these will align nicely
      \parbox{1.6cm}{\centering 4DGS-1\\\cite{yang2023gs4d}} & 
      \parbox{1.6cm}{\centering 4DGS-2\\\cite{wu20244d}} & 
      \parbox{1.6cm}{\centering Ex4DGS\\\cite{lee2024fully}} & 
      \parbox{1.6cm}{\centering FTGS\\\cite{wang2025freetimegs}} & 
      \parbox{1.6cm}{\centering \textbf{GraphiGS}\\\textbf{(Ours)}} & 
      \parbox{1.6cm}{\centering \textbf{GraphiTS}\\\textbf{(Ours)}} \\[5pt]
      
      % --- Row 1: Crop A ---
      % Width 0.163 fills the 6-column space perfectly (6 * 0.163 ~ 0.98)
      \includegraphics[width=0.163\linewidth]{#1/4dgs_iclr_a.png} &
      \includegraphics[width=0.163\linewidth]{#1/4dgs_cvpr_a.png} &
      \includegraphics[width=0.163\linewidth]{#1/ex4dgs_a.png} &
      \includegraphics[width=0.163\linewidth]{#1/ftgs_a.png} &
      \includegraphics[width=0.163\linewidth]{#1/graphigs_a.png} &
      \includegraphics[width=0.163\linewidth]{#1/graphits_a.png} \\[1pt]

      % --- Row 2: Crop B ---
      \includegraphics[width=0.163\linewidth]{#1/4dgs_iclr_b.png} &
      \includegraphics[width=0.163\linewidth]{#1/4dgs_cvpr_b.png} &
      \includegraphics[width=0.163\linewidth]{#1/ex4dgs_b.png} &
      \includegraphics[width=0.163\linewidth]{#1/ftgs_b.png} &
      \includegraphics[width=0.163\linewidth]{#1/graphigs_b.png} &
      \includegraphics[width=0.163\linewidth]{#1/graphits_b.png} \\
      
    \end{tabular}
  \end{minipage}
}

\newcommand{\figrowCropsTwoRowWL}[5]{%
  % Configuration
  \setlength{\tabcolsep}{0pt} % We control spacing manually with @{\hspace{...}}
  \renewcommand{\arraystretch}{0.5} % Keep text tight
  
  % --- Internal Helpers for Vertical Centering ---
  % Wraps image in a box aligned at its vertical center
  \def\vcimg##1{\parbox[c]{0.153\linewidth}{\includegraphics[width=\linewidth]{##1}}}%
  % Wraps label in a box aligned at its vertical center
  \def\vclbl##1{\parbox[c]{1em}{\centering\rotatebox{90}{\scriptsize \textbf{##1}}}}%
  
  % --- Left Block: Full Ground Truth (Unchanged) ---
  \begin{minipage}[c]{0.28\linewidth} 
    \centering
    % Label in 2 lines to match the height of headers on the right
    \parbox{2.5cm}{\centering \scriptsize \textbf{Ground}\\\textbf{Truth}} \par\vspace{3pt}
    \includegraphics[width=\linewidth]{#1/gt.png}
  \end{minipage}%
  \hfill % Push grid to right
  % --- Right Block: Labels + 6 Columns of Methods ---
  \begin{minipage}[c]{0.71\linewidth}
    \centering
    \tiny % Use tiny text to fit method names
    % 7 columns: 1 label column + 6 method columns
    \begin{tabular}{@{}c@{\hspace{2pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{}}
      % --- Header Row: Method Names ---
      &
      \parbox{1.6cm}{\centering 4DGS-1\\\cite{yang2023gs4d}} & 
      \parbox{1.6cm}{\centering 4DGS-2\\\cite{wu20244d}} & 
      \parbox{1.6cm}{\centering Ex4DGS\\\cite{lee2024fully}} & 
      \parbox{1.6cm}{\centering FTGS\\\cite{wang2025freetimegs}} & 
      \parbox{1.6cm}{\centering \textbf{GraphiGS}\\\textbf{(Ours)}} & 
      \parbox{1.6cm}{\centering \textbf{GraphiTS}\\\textbf{(Ours)}} \\[5pt]
      
      % --- Row 1: Crop A ---
      \vclbl{#4} &
      \vcimg{#1/4dgs_iclr_#2_a.png} &
      \vcimg{#1/4dgs_cvpr_#2_a.png} &
      \vcimg{#1/ex4dgs_#2_a.png} &
      \vcimg{#1/ftgs_#2_a.png} &
      \vcimg{#1/graphigs_#2_a.png} &
      \vcimg{#1/graphits_#2_a.png} \\
      \noalign{\vspace{1pt}} % Force exact 1pt vertical gap

      % --- Row 2: Crop B ---
      \vclbl{#5} &
      \vcimg{#1/4dgs_iclr_#3_a.png} &
      \vcimg{#1/4dgs_cvpr_#3_a.png} &
      \vcimg{#1/ex4dgs_#3_a.png} &
      \vcimg{#1/ftgs_#3_a.png} &
      \vcimg{#1/graphigs_#3_a.png} &
      \vcimg{#1/graphits_#3_a.png} \\
      
    \end{tabular}
  \end{minipage}
}

\newcommand{\figrowCropsThreeRowWL}[7]{%
  % Configuration
  \setlength{\tabcolsep}{0pt} % We control spacing manually with @{\hspace{...}}
  \renewcommand{\arraystretch}{0.5} % Keep text tight
  
  % --- Internal Helpers for Vertical Centering ---
  % Wraps image in a box aligned at its vertical center
  \def\vcimg##1{\parbox[c]{0.153\linewidth}{\includegraphics[width=\linewidth]{##1}}}%
  % Wraps label in a box aligned at its vertical center
  \def\vclbl##1{\parbox[c]{1em}{\centering\rotatebox{90}{\scriptsize \textbf{##1}}}}%
  
  % --- Left Block: Full Ground Truth ---
  \begin{minipage}[c]{0.28\linewidth} 
    \centering
    \parbox{2.5cm}{\centering \scriptsize \textbf{Ground}\\\textbf{Truth}} \par\vspace{3pt}
    \includegraphics[width=\linewidth]{#1/gt.png}
  \end{minipage}%
  \hfill % Push grid to right
  % --- Right Block: Labels + 6 Columns of Methods ---
  \begin{minipage}[c]{0.71\linewidth}
    \centering
    \tiny % Use tiny text to fit method names
    % 7 columns: Label + 1pt Gap + Method + 1pt Gap + Method ...
    \begin{tabular}{@{}c@{\hspace{2pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{}}
      % --- Header Row ---
      &
      \parbox{1.6cm}{\centering 4DGS-1\\\cite{yang2023gs4d}} & 
      \parbox{1.6cm}{\centering 4DGS-2\\\cite{wu20244d}} & 
      \parbox{1.6cm}{\centering Ex4DGS\\\cite{lee2024fully}} & 
      \parbox{1.6cm}{\centering FTGS\\\cite{wang2025freetimegs}} & 
      \parbox{1.6cm}{\centering \textbf{GraphiGS}\\\textbf{(Ours)}} & 
      \parbox{1.6cm}{\centering \textbf{GraphiTS}\\\textbf{(Ours)}} \\[5pt]
      
      % --- Row 1: Crop A ---
      \vclbl{#5} &
      \vcimg{#1/4dgs_iclr_#2_a.png} &
      \vcimg{#1/4dgs_cvpr_#2_a.png} &
      \vcimg{#1/ex4dgs_#2_a.png} &
      \vcimg{#1/ftgs_#2_a.png} &
      \vcimg{#1/graphigs_#2_a.png} &
      \vcimg{#1/graphits_#2_a.png} \\
      \noalign{\vspace{1pt}} % Force exact 1pt vertical gap

      % --- Row 2: Crop B ---
      \vclbl{#6} &
      \vcimg{#1/4dgs_iclr_#3_a.png} &
      \vcimg{#1/4dgs_cvpr_#3_a.png} &
      \vcimg{#1/ex4dgs_#3_a.png} &
      \vcimg{#1/ftgs_#3_a.png} &
      \vcimg{#1/graphigs_#3_a.png} &
      \vcimg{#1/graphits_#3_a.png} \\
      \noalign{\vspace{1pt}} % Force exact 1pt vertical gap

      % --- Row 3: Crop C ---
      \vclbl{#7} &
      \vcimg{#1/4dgs_iclr_#4_a.png} &
      \vcimg{#1/4dgs_cvpr_#4_a.png} &
      \vcimg{#1/ex4dgs_#4_a.png} &
      \vcimg{#1/ftgs_#4_a.png} &
      \vcimg{#1/graphigs_#4_a.png} &
      \vcimg{#1/graphits_#4_a.png} \\
      
    \end{tabular}
  \end{minipage}
}

\newcommand{\figrowCropsTwoRowWLShort}[5]{%
  % Configuration
  \setlength{\tabcolsep}{0pt} % We control spacing manually with @{\hspace{...}}
  \renewcommand{\arraystretch}{0.5} % Keep text tight
  
  % --- Internal Helpers for Vertical Centering ---
  % Increased width to 0.235 to fill space with only 4 images
  \def\vcimg##1{\parbox[c]{0.21\linewidth}{\includegraphics[width=\linewidth]{##1}}}%
  \def\vclbl##1{\parbox[c]{1em}{\centering\rotatebox{90}{\scriptsize \textbf{##1}}}}%
  
  % --- Left Block: Full Ground Truth ---
  \begin{minipage}[c]{0.28\linewidth} 
    \centering
    \parbox{2.5cm}{\centering \scriptsize \textbf{Ground}\\\textbf{Truth}} \par\vspace{3pt}
    \includegraphics[width=\linewidth]{#1/gt.png}
  \end{minipage}%
  \hfill % Push grid to right
  % --- Right Block: Labels + 4 Columns of Methods ---
  \begin{minipage}[c]{0.71\linewidth}
    \centering
    \tiny % Use tiny text to fit method names
    % 5 columns: 1 label column + 4 method columns
    \begin{tabular}{@{}c@{\hspace{2pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{}}
      % --- Header Row ---
      % Parbox width increased to 2.5cm to match larger image width
      &
      \parbox{2.5cm}{\centering W/O Upgrade} & 
      \parbox{2.5cm}{\centering W Upgrade} & 
      \parbox{2.5cm}{\centering W/O Upgrade} & 
      \parbox{2.5cm}{\centering W Upgrade} \\[5pt]
      
      % --- Row 1: Crop A ---
      % Uses #2 for filename suffix, #4 for Label
      \vclbl{#4} &
      \vcimg{#1/ftgs_#2_a.png} &
      \vcimg{#1/upgrade_#2_a.png} &
      \vcimg{#1/ftgs_#2_b.png} &
      \vcimg{#1/upgrade_#2_b.png} \\
      \noalign{\vspace{1pt}} % Force exact 1pt vertical gap

      % --- Row 2: Crop B ---
      % Uses #3 for filename suffix, #5 for Label
      \vclbl{#5} &
      \vcimg{#1/ftgs_#3_a.png} &
      \vcimg{#1/upgrade_#3_a.png} &
      \vcimg{#1/ftgs_#3_b.png} &
      \vcimg{#1/upgrade_#3_b.png} \\
      
    \end{tabular}
  \end{minipage}
}

% \newcommand{\figrowCropsTwoRowWLShortAbl_old}[5]{%
%   % Configuration
%   \setlength{\tabcolsep}{0pt} 
%   \renewcommand{\arraystretch}{0.5} 
  
%   % --- Internal Helpers for Vertical Centering ---
%   % Grid images set to 0.30 to represent ~30% of the RIGHT block (making them small)
%   \def\vcimg##1{\parbox[c]{0.30\linewidth}{\includegraphics[width=\linewidth]{##1}}}%
%   \def\vclbl##1{\parbox[c]{1em}{\centering\rotatebox{90}{\scriptsize \textbf{##1}}}}%
  
%   % --- CENTERING WRAPPER ---
%   \centering
  
%   % --- Left Block: Ground Truth (Restored to Large Size) ---
%   \begin{minipage}[c]{0.28\linewidth} 
%     \centering
%     \parbox{2.5cm}{\centering \scriptsize \textbf{Ground}\\\textbf{Truth}} \par\vspace{3pt}
%     \includegraphics[width=\linewidth]{#1/gt.png}
%   \end{minipage}%
%   \hspace{4pt}% Small fixed gap
%   % --- Right Block: 3 Methods (Constrained Width) ---
%   \begin{minipage}[c]{0.60\linewidth}
%     \centering
%     \tiny 
%     \begin{tabular}{@{}c@{\hspace{2pt}}c@{\hspace{2pt}}c@{\hspace{2pt}}c@{}}
%       % --- Header Row ---
%       % Headers match the image width (0.30)
%       &
%       \parbox{0.30\linewidth}{\centering W/O Higher Order Dynamics} & 
%       \parbox{0.30\linewidth}{\centering W/O $P(\alpha \mid \theta, C, T)$} & 
%       \parbox{0.30\linewidth}{\centering \textbf{GraphiTS (Ours)}} \\[5pt]
      
%       % --- Row 1: Crop A ---
%       \vclbl{#4} &
%       \vcimg{#1/no_higher_#2_a.png} &
%       \vcimg{#1/no_likeli_#2_a.png} &
%       \vcimg{#1/graphits_#2_a.png} \\
%       \noalign{\vspace{1pt}} 

%       % --- Row 2: Crop B ---
%       \vclbl{#5} &
%       \vcimg{#1/no_higher_#3_a.png} &
%       \vcimg{#1/no_likeli_#3_a.png} &
%       \vcimg{#1/graphits_#3_a.png} \\
      
%     \end{tabular}
%   \end{minipage}
% }

\newcommand{\figrowCropsTwoRowWLShortAbl}[5]{%
  % Configuration
  \setlength{\tabcolsep}{0pt} % We control spacing manually with @{\hspace{...}}
  \renewcommand{\arraystretch}{0.5} % Keep text tight
  
  % --- Internal Helpers for Vertical Centering ---
  % Increased width to 0.235 to fill space with only 4 images
  \def\vcimg##1{\parbox[c]{0.21\linewidth}{\includegraphics[width=\linewidth]{##1}}}%
  \def\vclbl##1{\parbox[c]{1em}{\centering\rotatebox{90}{\scriptsize \textbf{##1}}}}%
  
  % --- Left Block: Full Ground Truth ---
  \begin{minipage}[c]{0.28\linewidth} 
    \centering
    \parbox{2.5cm}{\centering \scriptsize \textbf{Ground}\\\textbf{Truth}} \par\vspace{3pt}
    \includegraphics[width=\linewidth]{#1/gt.png}
  \end{minipage}%
  \hfill % Push grid to right
  % --- Right Block: Labels + 4 Columns of Methods ---
  \begin{minipage}[c]{0.71\linewidth}
    \centering
    \tiny % Use tiny text to fit method names
    % 5 columns: 1 label column + 4 method columns
    \begin{tabular}{@{}c@{\hspace{2pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{}}
      % --- Header Row ---
      % Parbox width increased to 2.5cm to match larger image width
      &
      \parbox{2.5cm}{\centering W/O Higher\\Order Dynamics} & 
      \parbox{2.5cm}{\centering W/O $P(\alpha \mid \theta, C, T)$} & 
      \parbox{2.5cm}{\centering W/O\\Stochasticity} & 
      \parbox{2.5cm}{\centering \textbf{GraphiTS (Ours)}} \\[5pt]
      
      % --- Row 1: Crop A ---
      \vclbl{#4} &
      \vcimg{#1/no_higher_#2_a.png} &
      \vcimg{#1/no_likeli_#2_a.png} &
      \vcimg{#1/deterministic_#2_a.png} &
      \vcimg{#1/graphits_#2_a.png} \\
      \noalign{\vspace{1pt}} % Force exact 1pt vertical gap

      % --- Row 2: Crop B ---
      \vclbl{#5} &
      \vcimg{#1/no_higher_#3_a.png} &
      \vcimg{#1/no_likeli_#3_a.png} &
      \vcimg{#1/deterministic_#3_a.png} &
      \vcimg{#1/graphits_#3_a.png} \\
      
    \end{tabular}
  \end{minipage}
}
